RLP: Reinforcement as a Pretraining Objective

The dominant paradigm for training large reasoning models starts with pre-training using next-token prediction loss on vast amounts of data. Reinforcement learning, while powerful in scaling reasoning, is introduced only as the very last phase of post-training, preceded by supervised fine-tuning. While dominant, is this an optimal way of training? In this paper, we present RLP, an information-driven reinforcement pretraining objective, that brings the core spirit of reinforcement learning -- exploration -- to the last phase of pretraining. The key idea is to treat chain-of-thought as an exploratory action, with rewards computed based on the information gain it provides for predicting future tokens. This training objective essentially encourages the model to think for itself before predicting what comes next, thus teaching an independent thinking behavior earlier in the pretraining. More concretely, the reward signal measures the increase in log-likelihood of the next token when conditioning on both context and a sampled reasoning chain, compared to conditioning on context alone. This approach yields a verifier-free dense reward signal, allowing for efficient training for the full document stream during pretraining. Specifically, RLP reframes reinforcement learning for reasoning as a pretraining objective on ordinary text, bridging the gap between next-token prediction and the emergence of useful chain-of-thought reasoning. Pretraining with RLP on Qwen3-1.7B-Base lifts the overall average across an eight-benchmark math-and-science suite by 19%. With identical post-training, the gains compound, with the largest improvements on reasoning-heavy tasks such as AIME25 and MMLU-Pro. Applying RLP to the Nemotron-Nano-12B-v2 increases the overall average from 42.81% to 61.32% and raises the average on scientific reasoning by 23%, demonstrating scalability across architectures and model sizes.

==> sections/results_backup.tex <==
\section{Results}
\label{sec:results}

We compare \mours with \mbase and \mcpt before and after doing post-training for the \qwen in Table \ref{tab:qwen-main-res}.
We see that \mours is on average 19\% and 17\% better than \mbase and \mcpt respectively. In addition, we also run the post-training pipeline on all three of the models and find that \mours is on average 8\% and 7\% better than \mbase and \mcpt respectively after post-training.
This 
%not only shows that post-training does not wash off the gains from using \ours during pre-training, but also 
shows that post-training \mours pushes the reasoning skills even further.

\begin{table}[htbp]
\centering
\sisetup{table-format=2.2}
% \begin{tabular}{l *{6}{S[table-format=2.2]}}
\begin{tabular}{l
      S
      S
      >{\bfseries\columncolor{gray!8}}S
      S
      S
      >{\bfseries\columncolor{gray!15}}S}
\toprule
% \textbf{Benchmark} & \textbf{Base} & \textbf{+CPT} & \textbf{+\ours} & \textbf{+Post} & \textbf{+CPT+Post} & \textbf{+\ours+Post} \\
\textbf{Benchmark} & \mbase & \mcpt & \mours & \textbf{\mbase+Post} & \textbf{\mcpt+Post} & \textbf{\mours+Post} \\
\midrule
AIME25              & 2.25  & 3.96  & 5.02  & 5.32  & 5.89  & 7.05  \\
MATH500            & 48.45 & 57.52 & 58.48 & 61.92 & 62.70 & 64.30 \\
GSM8K               & 54.16 & 72.85 & 74.48 & 78.22 & 78.70 & 80.50 \\
AMC23               & 25.94 & 31.25 & 31.25 & 35.00 & 34.38 & 36.50 \\
Minerva                & 15.30 & 19.03 & 21.19 & 25.30 & 26.10 & 27.80 \\
MMLU                & 50.08 & 41.95 & 56.14 & 58.36 & 59.00 & 61.50 \\
MMLU@1[4]           & 44.85 & 40.00 & 52.18 & 56.00 & 58.53 & 61.00 \\
MMLU-Pro            & 28.17 & 27.81 & 34.62 & 37.85 & 39.92 & 42.40 \\
MMLU-Pro@1[4]       & 23.95 & 24.61 & 30.80 & 36.53 & 38.49 & 41.30 \\
GPQA                & 25.25 & 26.26 & 28.28 & 30.93 & 29.27 & 33.33 \\
GPQA@1[4]           & 27.52 & 24.75 & 27.02 & 31.52 & 30.01 & 34.97 \\
% \cmidrule(r){1-1} \cmidrule(l){2-7}
\midrule
Math Avg            & 24.35 & 30.77 & 31.74 & 34.29 & 34.63 & 36.03 \\
Science Avg         & 34.50 & 32.01 & 39.68 & 42.38 & 42.73 & 45.74 \\
Science Avg@1[4]    & 32.11 & 29.79 & 36.67 & 41.35 & 42.34 & 45.76 \\
% \cmidrule(r){1-1} \cmidrule(l){2-7}
\midrule
\textbf{Overall Avg}& 30.32 & 30.85 & \bfseries 36.03 & 39.34 & 39.90 & \bfseries 42.51 \\
\bottomrule
\end{tabular}
\caption{Quantitative benchmarks for Qwen3-1.7B-Base experiments, underscoring the impact of RLPT. Shaded columns represent RLPT variants. Post variants include SFT + RLVR post training.}
\label{tab:qwen-main-res}
\end{table}

\paragraph{Scaling to Larger Model Size and Different Architecture:} We further scale \ours to \nemo \citep{nano2025efficient}. It is a hybrid Mamba-Transformer language model of 12B parameter size. 
In this comparison we take a checkpoint of \nemo trained till $19.8$ trillion tokens and apply \ours for $250$ million tokens only.
\mbase on the other hand is trained for $20$ trillion tokens.
Table~\ref{tab:nano12b-comp} shows the results of \mbase and \mours for \nemo and it demonstrates that \ours scales effectively with model size and across model architectures.
Specifically, \mours is relatively $35$\% on average better than \mbase inspite of being trained on approx. $200$ billion less tokens.
In particular, the science benchmarks benefit heavily from \ours which shows the generalizability of \ours to induce reasoning beyond math domain.
\begin{wraptable}[9]{r}{0.7\textwidth}
\centering
\vspace{8mm}
\resizebox{0.7\textwidth}{!}{% 
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Model} & \textbf{\shortstack{Math Avg@1[8]}} & \textbf{Science Avg} & \textbf{\shortstack{Science Avg@1[4]}} 	& \textbf{Avg}\\\toprule
\mbase & 61.38 & 34.51 & 32.54 & 42.81 \\ 
\mours &  \textbf{65.33} & \textbf{57.26} & \textbf{61.37} & \textbf{61.32} \\
\toprule
\end{tabular}
}
\caption{\textbf{Comparison of BASE and \ours for the \nemo model}}
\label{tab:nano12b-comp}
\end{wraptable} 


% \begin{table}[htbp]
% \centering
% \sisetup{table-format=2.2}
% % \begin{tabular}{l *{6}{S[table-format=2.2]}}
% \begin{tabular}{l
%       S
%       S
%       >{\bfseries\columncolor{gray!8}}S
%       S
%       S
%       >{\bfseries\columncolor{gray!15}}S}
% \toprule
% \textbf{Benchmark} & \textbf{Base} & \textbf{+CPT} & \textbf{+\ours} & \textbf{+Post} & \textbf{+CPT+Post} & \textbf{+\ours+Post} \\
% \midrule
% AIME25              & 2.25  & 3.96  & 5.02  & 5.32  & 5.89  & 7.05  \\
% MATH500            & 48.45 & 57.52 & 58.48 & 61.92 & 62.70 & 64.30 \\
% GSM8K               & 54.16 & 72.85 & 74.48 & 78.22 & 78.70 & 80.50 \\
% AMC23               & 25.94 & 31.25 & 31.25 & 35.00 & 34.38 & 36.50 \\
% Minerva                & 15.30 & 19.03 & 21.19 & 25.30 & 26.10 & 27.80 \\
% MMLU                & 50.08 & 41.95 & 56.14 & 58.36 & 59.00 & 61.50 \\
% MMLU@1[4]           & 44.85 & 40.00 & 52.18 & 56.00 & 58.53 & 61.00 \\
% MMLU-Pro            & 28.17 & 27.81 & 34.62 & 37.85 & 39.92 & 42.40 \\
% MMLU-Pro@1[4]       & 23.95 & 24.61 & 30.80 & 36.53 & 38.49 & 41.30 \\
% GPQA                & 25.25 & 26.26 & 28.28 & 30.93 & 29.27 & 33.33 \\
% GPQA@1[4]           & 27.52 & 24.75 & 27.02 & 31.52 & 30.01 & 34.97 \\
% % \cmidrule(r){1-1} \cmidrule(l){2-7}
% \midrule
% Math Avg            & 24.35 & 30.77 & 31.74 & 34.29 & 34.63 & 36.03 \\
% Science Avg         & 34.50 & 32.01 & 39.68 & 42.38 & 42.73 & 45.74 \\
% Science Avg@1[4]    & 32.11 & 29.79 & 36.67 & 41.35 & 42.34 & 45.76 \\
% % \cmidrule(r){1-1} \cmidrule(l){2-7}
% \midrule
% \textbf{Overall Avg}& 30.32 & 30.85 & \bfseries 36.03 & 39.34 & 39.90 & \bfseries 42.51 \\
% \bottomrule
% \end{tabular}
% \caption{Quantitative benchmarks for \texttt{Qwen3-1.7B-Base} experiments, underscoring the impact of RLPT. Shaded columns represent RLPT variants.}
% \label{tab:qwen-main-res}
% \end{table}

% \shrimai{Add Code evaluations}

% \begin{table}[t]
%   \centering
%   \small
%   \setlength{\tabcolsep}{6pt}
%   \renewcommand{\arraystretch}{1.12}
%   \begin{threeparttable}
%     \caption{Quantitative benchmarks for \texttt{Qwen3-1.7B-Base} experiments, underscoring the impact of RLPT. Shaded columns represent RLPT variants.}
%     \label{tab:diverse_data_qwen}

%     \begin{tabular}{
%       l
%       S
%       S
%       S
%       S
%       >{\columncolor{gray!8}}S
%       >{\bfseries\columncolor{gray!15}}S
%     }
%       \toprule
%       & \multicolumn{4}{c}{\textbf{No RLPT}} & \multicolumn{2}{c}{\textbf{RLPT}} \\
%       \cmidrule(lr){2-5}\cmidrule(l){6-7}
%       \textbf{Benchmark}
%         & \textbf{Base} & \textbf{+CPT} & \textbf{+Post}\tnote{a} & \textbf{+CPT+Post}\tnote{a}
%         & \textbf{+RLPT} & \textbf{+RLPT+Post}\tnote{a} \\
%       \midrule
%       Math-500             & 48.45 & 57.52 & 61.92 & 62.70 & 58.48 & 64.30 \\
%       GSM8k                & 54.16 & 72.85 & 78.22 & 78.70 & 74.48 & 80.50 \\
%       AIME25               &  2.25 &  3.96 &  5.32 &  5.89 &  5.02 &  7.05 \\
%       AMC23                & 25.94 & 31.25 & 35.00 & 34.38 & 31.25 & 36.50 \\
%       Minerva                 & 15.30 & 19.03 & 25.30 & 26.10 & 21.19 & 27.80 \\
%       MMLU                 & 50.08 & 41.95 & 58.36 & 59.00 & 56.14 & 61.50 \\
%       MMLU@1[4]            & 44.85 & 40.00 & 56.00 & 58.53 & 52.18 & 61.00 \\
%       MMLU-Pro             & 28.17 & 27.81 & 37.85 & 39.92 & 34.62 & 42.40 \\
%       MMLU-Pro@1[4]        & 23.95 & 24.61 & 36.53 & 38.49 & 30.80 & 41.30 \\
%       GPQA                 & 25.25 & 26.26 & 30.93 & 29.27 & 28.28 & 33.33 \\
%       GPQA@1[4]            & 27.52 & 24.75 & 31.52 & 30.01 & 27.02 & 34.97 \\
%       \midrule
%       Math Avg.             & 24.35 & 30.77 & 34.29 & 34.63 & 31.74 & 36.03 \\
%       Science Avg.          & 34.50 & 32.01 & 42.38 & 42.73 & 39.68 & 45.74 \\
%       Science Avg@1[4]     & 32.11 & 29.79 & 41.35 & 42.34 & 36.67 & 45.76 \\
%       \midrule
%       \textbf{Overall} & \bfseries 30.32 & \bfseries 30.85 & \bfseries 39.34 & \bfseries 39.90 & \bfseries 36.03 & \bfseries 42.51 \\
%       \bottomrule
%     \end{tabular}

%     \begin{tablenotes}[flushleft]
%       \footnotesize
%       \item[a] Post variants include optimized SFT + RLVR post training.
%     \end{tablenotes}
%   \end{threeparttable}
% \end{table}


% \shrimai{Thought: when we present results for Nano model, we should also highlight the generalizability of our technique across model architectures - nano is a hybrid mamba 2 based model.}

\paragraph{RPT Comparison}


Following the experimental setup in RPT with Omni‑MATH dataset, we trained both methods for one epoch under matched data and compute budgets before evaluating on our benchmark suite. As summarized in Table \autoref{tab:nano_comp}, \ours{} achieves uniformly higher aggregates: \emph{Math Avg} improves from 47.50 to 49.62 (+2.12; +4.5\% relative), \emph{Science Avg} from 35.88 to 37.07 (+1.19; +3.3\%), and \emph{Overall Avg} from 41.69 to 43.35 (+1.66; +4.0\%). Methodologically, RPT applies reinforcement only to tokens pre‑selected by an auxiliary assistant via entropy filtering and optimizes a sparse, binary next‑token correctness signal that ignores the CoT content, limiting where the signal can be applied. In contrast, \ours{} evaluates each sampled CoT by the

\begin{wraptable}{r}{0.55\linewidth}
\vspace{-8pt}
\centering
\footnotesize
\setlength{\tabcolsep}{6pt}
\begin{tabular}{l
                S[table-format=2.2]
                S[table-format=2.2]
                S[table-format=2.2]}
\toprule
\textbf{Model} & \textbf{Math Avg} & \textbf{Science Avg} & \textbf{Overall Avg} \\
\midrule
\mbase           & 35.96 & 32.11 & 34.03 \\
\mrpt           & 47.50 & 35.88 & 41.69 \\
\rowcolor{gray!15}
\textbf{\mours{}} & \bfseries 49.62 & \bfseries 37.07 & \bfseries 43.35 \\
\addlinespace[2pt]
\bottomrule
\end{tabular}
\caption{\textbf{\ours{} outperforms RPT across all averages.} \qwen was trained with both RPT and \ours{} for one epoch with matched data and compute.}
\vspace{-6pt}
\label{tab:nano_comp}
\end{wraptable} 

information gain it provides for the observed next token and updates at all positions without an auxiliary filter which yields consistently better averages under the matched setting above. Crucially, this dense, per‑token information‑gain reward supplies richer credit assignment than RPT’s sparse binary signal and, in our matched experiments, empirically yields better performance.




% \begin{table}[htbp]
% \centering
% \sisetup{table-format=2.2}
% \begin{tabular}{l *{6}{S[table-format=2.2]}}
% \toprule
% \textbf{Benchmark} & \textbf{Base} & \textbf{+RLPT1} & \textbf{+RLPT2} & \multicolumn{1}{c}{\textbf{+Post}} & \multicolumn{1}{c}{\textbf{+RLPT1+Post}} & \multicolumn{1}{c}{\textbf{+RLPT2+Post}} \\
% %& & & & & \multicolumn{1}{c}{\textbf{+Post}} & \multicolumn{1}{c}{\textbf{+Post}} \\
% %& & & & \multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{+RLVR}} & \multicolumn{1}{c}{\textbf{+RLVR}} \\
% \midrule
% AIME25              &   \\
% MATH500             & 79.95 & 72.10 & \\
% GSM8K               & 72.31 & 91.25\\
% AMC23               & 70.63 & 48.75 \\
% Minerva             & 22.61 & 32.44 \\
% MMLU                & 54.12 & 69.43 \\
% MMLU@1[4]           & 48.01 & 68.13 \\
% MMLU-Pro            & 24.16 & 50.87 \\
% MMLU-Pro@1[4]       & 27.13 & 49.73 \\
% GPQA                & 25.25 & 37.88 \\
% GPQA@1[4]           & 22.47 & 32.32 \\
% \midrule
% Math Avg            &  \\
% Science Avg         & 34.51 & 52.73 \\
% Science Avg@1[4]    & 32.54 & 50.06 \\
% \midrule
% \textbf{Overall Avg}&  \\
% \bottomrule
% \end{tabular}
% \caption{Benchmark results for Nano-12B-Base and its training variants.}
% \label{tab:nano-main-results}
% \end{table}



